A fast solver for spectral element approximation applied to fractional differential equations using hierarchical matrix approximation

We develop a fast solver for the spectral element method (SEM) applied to the two-sided fractional diffusion equation on uniform, geometric and graded meshes. By approximating the singular kernel with a degenerate kernel, we construct a hierarchical matrix (H-matrix) to represent the stiffness matrix of the SEM and provide error estimates verified numerically. We can solve efficiently the H-matrix approximation problem using a hierarchical LU decomposition method, which reduces the computational cost to $O(R^2 N_d \log^2N) +O(R^3 N_d \log N)$, where $R$ it is the rank of submatrices of the H-matrix approximation, $N_d$ is the total number of degrees of freedom and $N$ is the number of elements. However, we lose the high accuracy of the SEM. Thus, we solve the corresponding preconditioned system by using the H-matrix approximation problem as a preconditioner, recovering the high order accuracy of the SEM. The condition number of the preconditioned system is independent of the polynomial degree $P$ and grows with the number of elements, but at modest values of the rank $R$ is below order 10 in our experiments, which represents a reduction of more than 11 orders of magnitude from the unpreconditioned system; this reduction is higher in the two-sided fractional derivative compared to one-sided fractional derivative. The corresponding cost is $O(R^2 N_d \log^2 N)+O(R^3 N_d \log N)+O(N_d^2)$. Moreover, by using a structured mesh (uniform or geometric mesh), we can further reduce the computational cost to $O(R^2 N_d\log^2 N) +O(R^3 N_d \log N)+ O(P^2 N\log N)$ for the preconditioned system. We present several numerical tests to illustrate the proposed algorithm using $h$ and $p$ refinements.

==> Fast_Solver_SEM_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{caption2}
\usepackage{psfrag}
\usepackage{amsmath}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{bm}   %
\usepackage{float}
\usepackage{latexsym}
\usepackage{lscape}
\usepackage{mathrsfs}
\usepackage{verbatim}
%\usepackage{showlabels}
\usepackage{appendix}
\usepackage{tikz}
\allowdisplaybreaks[4]
%\usepackage{subfigure}
\newtheorem{remark}{Remark}[section]
\newtheorem{thm}{Theorem}
%\newtheorem{proof}{Proof}
%\newtheorem{definition}{Definition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{exam}{Example}
%\newproof{pf}{Proof}
\newcommand{\ds}{\displaystyle}
\newcommand{\f}{\frac}
\newcommand{\om}{\Omega}
\newcommand{\p}{\partial}


\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bex}{\begin{eqnarray*}}
\newcommand{\eex}{\end{eqnarray*}}
\newcommand{\be}{\begin{equation*}}
\newcommand{\ee}{\end{equation*}}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}


\def\br{\begin{eqnarray}}
\def\er{\end{eqnarray}}
\def\brr{\bq\begin{array}{rlll}}
\def\err{\end{array}\eq}
\def\no{\nonumber}
\def\N{{\mathbb {N} }}

\def\d{{\mathrm {d} }}




\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A fast solver for spectral element approximation applied to fractional differential equations using hierarchical matrix approximation}
\newcommand{\TheAuthors}{Xianjuan Li and Zhiping Mao and Fangying Song and Hong Wang and George Em Karniadakis}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{This work was supported by the MURI/ARO on ``Fractional PDEs for Conservation Laws and Beyond: Theory, Numerics and Applications" (W911NF-15-1-0562).} The research of the first author was partially supported by NSF of China
(11771083, 61672005), NSF of Fujian Province (2016J01013).
}


\author{
  Xianjuan Li\footnotemark[2]
  \and
  Zhiping Mao\footnotemark[3] \footnotemark[5]
  \and
  Fangying Song\footnotemark[3]
  \and
  Hong Wang\footnotemark[4]
  \and
  George Em Karniadakis\footnotemark[3]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}



%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

